Predicting Terrorist Attacks in the United States using Localized News Data

Terrorism is a major problem worldwide, causing thousands of fatalities and billions of dollars in damage every year. Toward the end of better understanding and mitigating these attacks, we present a set of machine learning models that learn from localized news data in order to predict whether a terrorist attack will occur on a given calendar date and in a given state. The best model--a Random Forest that learns from a novel variable-length moving average representation of the feature space--achieves area under the receiver operating characteristic scores $> .667$ on four of the five states that were impacted most by terrorism between 2015 and 2018. Our key findings include that modeling terrorism as a set of independent events, rather than as a continuous process, is a fruitful approach--especially when the events are sparse and dissimilar. Additionally, our results highlight the need for localized models that account for differences between locations. From a machine learning perspective, we found that the Random Forest model outperformed several deep models on our multimodal, noisy, and imbalanced data set, thus demonstrating the efficacy of our novel feature representation method in such a context. We also show that its predictions are relatively robust to time gaps between attacks and observed characteristics of the attacks. Finally, we analyze factors that limit model performance, which include a noisy feature space and small amount of available data. These contributions provide an important foundation for the use of machine learning in efforts against terrorism in the United States and beyond.

==> related.tex <==
% \section{Related Work} \label{sec:related}



% %% Notes

%  \cite{johnson2015modeling} Assumes acts of terrorism are part of a ``terrorist campaign'' or ongoing conflict. Seeks to model the progression of human violence. ``Given that human
% conflicts and terror campaigns are examples of a highly complex dynamical system
% driven by interconnected issues and actors, we demonstrate in this chapter that a
% potentially fruitful approach lies within the framework of the statistical physics of
% non-equilibrium open systems.''

% This new one: \cite{li2019longrange} - acknowledges event predictions are not good. ``Terrorism is essentially an unstable system of interdependent events where small perturbations might be catastrophic.''---maybe true for following organizations, etc., but not really for our case. Assume crime is a network that follows certain spatiotemporal patterns. Can we assume the same for terrorism? They utilize the same framework for predicting crime in Chicago to terrorism in the middle east. Would not address the challenges faced by our problem.


% On Bayesian spatial dynamics of lethal events - related work is very helpful \cite{python2019bayesian}. ``We assume that the characteristics of terrorism under consideration—lethality of
% terrorism, severity, and frequency of lethal terrorist attacks—are continuous phenomena with Gaussian properties, which exhibit dependencies in both space and time.''
% ``Terrorist attacks occur at specific locations on earth and are therefore inherently
% discrete. However, we consider three characteristics of terrorism: potential to kill
% (lethality L), number of deadly victims (severity S), and the number of lethal attacks
% (frequency F) as continuous phenomena (in the sense of geostatistics (Cressie, 1991)),
% which are observed at s locations (attacks) over the surface of the earth S
% 2 at time t ∈ R.''

% \cite{vanderzee2018predicting} - predicting the spread of terroritory controlled by ISIS using a graph approach.

% \cite{johnson2013particles} - describes the escalation of human violence as a dynamical spatiotemporal system, which exhibits patterns. 

% \cite{johnson2011pattern} - attempts to model how lethality of attacks escalates in spatiotemporal patterns. All in middle east.


% \begin{enumerate}
% \item Crime prediction: modeling [urban] crime as a diffusive process in space/time
% \item Terrorism prediction: borrows from crime prediction, focused in middle east, does not address event-level predictions, generally focused on “spread”
% \item Terrorism detection: mostly social media
% \end{enumerate}

% We would be the first to treat terrorist events as stochastic. Makes sense in the U.S. where many events are not perpetrated by an organized movement (need to study further). Contributes both predictive power & a potentially new paradigm for studying terrorism.

% \cite{talreja2017terrorism} uses GTD to predict the group responsible for an attack.

%  \cite{johnson2015modeling} Assumes acts of terrorism are part of a ``terrorist campaign'' or ongoing conflict. Seeks to model the progression of human violence. ``Given that human
% conflicts and terror campaigns are examples of a highly complex dynamical system
% driven by interconnected issues and actors, we demonstrate in this chapter that a
% potentially fruitful approach lies within the framework of the statistical physics of
% non-equilibrium open systems.''

% This new one: \cite{li2019longrange} - acknowledges event predictions are not good. ``Terrorism is essentially an unstable system of interdependent events where small perturbations might be catastrophic.''---maybe true for following organizations, etc., but not really for our case. Assume crime is a network that follows certain spatiotemporal patterns. Can we assume the same for terrorism? They utilize the same framework for predicting crime in Chicago to terrorism in the middle east. Would not address the challenges faced by our problem.

% On Bayesian spatial dynamics of lethal events - related work is very helpful \cite{python2019bayesian}. ``We assume that the characteristics of terrorism under consideration—lethality of
% terrorism, severity, and frequency of lethal terrorist attacks—are continuous phenomena with Gaussian properties, which exhibit dependencies in both space and time.''
% ``Terrorist attacks occur at specific locations on earth and are therefore inherently
% discrete. However, we consider three characteristics of terrorism: potential to kill
% (lethality L), number of deadly victims (severity S), and the number of lethal attacks
% (frequency F) as continuous phenomena (in the sense of geostatistics (Cressie, 1991)),
% which are observed at s locations (attacks) over the surface of the earth S
% 2 at time t ∈ R.''

% \subsection{On Modeling Terrorism} 

% \cite{yang2019quantifying} - quantifies future lethality of terrorist organizations.

% \cite{vanderzee2018predicting} - predicting the spread of terroritory controlled by ISIS using a graph approach.

% \cite{johnson2013particles} - describes the escalation of human violence as a dynamical spatiotemporal system, which exhibits patterns. 

% \cite{johnson2011pattern} - attempts to model how lethality of attacks escalates in spatiotemporal patterns. All in middle east.

% SOCIAL UNREST / GDELT

% \cite{qiao2017predicting} use features from GDELT to predict anomalies in CAMEO code 14, which they consider an indicator of social unrest events. the same but using a HMM and in Southeast Asia, using anomalies in GDELT CAMEO code 14. Key assumption is that there is an escalation that can be detected by the news.

% \cite{galla2018predicting} uses features from GDELT to predict the occurrence of social unrest events in the United States. Treats it as as classification problem. Uses a moving average for lead time and prediction windows.

% \cite{tolan2015experimental} uses the GTD alone to predict the organization responsible for attacks. 

% \cite{agarwal2019comparison} use GTD and weather information to make predictions about internal features. ``The main objective was achieved by dividing theanalysis into various modules: 1) prediction of casualties; 2) consideration of various attributes for identification of successfulness of the attack using RF, SVM [8] and Dummy classifier; 3) Algorithms like Multinomial Naive Bayes (NB) and Logistic Regression (LR) were employed for prediction of terrorist groups and; 4) the study of correlation between the attributes, the K-Means [8] clustering was adopted to form the clusters.''

% \cite{dunning2020higher} uses similarity networks to identify similarities between responsible groups.



% \cite{bang2018predicting} uses a multimodal approach (political and economic data) to predict the number of attacks in a given country over a five-year period.

% \cite{ding2017understanding} - uses history in the GTD, geological, drug activity, etc. to predict the occurrence of an attack in a small geographical space. However, most of the data is stationary - so results are probably biased toward similar regions where activity is already high. Also, they consider whether an attack will occur in the entire year of 2015. 


% \cite{zhao2017modeling} utilize multimodal data to predict the level of crime, as a regression problem, within NYC. They use features from the multimodal sources to describe the environment, and learn a deep model tailored to each region in the environment.

% \cite{kang2017prediction} uses multimodal and location-context data to predict occurrence of crime in a particular point of space or time. ''One possible approach to solve this problem is accurately predicting the probability of crime occurrences at a given date and location by scrutinizing and modeling various previous data on criminal activities.''
